Strengthened Fault Tolerance in Byzantine Fault Tolerant Replication

Byzantine fault tolerant (BFT) state machine replication (SMR) is an important building block for constructing permissioned blockchain systems. In contrast to Nakamoto Consensus where any block obtains higher assurance as buried deeper in the blockchain, in BFT SMR, any committed block is secure has a fixed resilience threshold. In this paper, we investigate strengthened fault tolerance (SFT) in BFT SMR under partial synchrony, which provides gradually increased resilience guarantees (like Nakamoto Consensus) during an optimistic period when the network is synchronous and the number of Byzantine faults is small. Moreover, the committed blocks can tolerate more than one-third (up to two-thirds) corruptions even after the optimistic period. Compared to the prior best solution Flexible BFT which requires quadratic message complexity, our solution maintains the linear message complexity of state-of-the-art BFT SMR protocols and requires only marginal bookkeeping overhead. We implement our solution over the open-source Diem project, and give experimental results that demonstrate its efficiency under real-world scenarios.

==> backup.tex <==
\subsection{Comparison with FBFT~\cite{malkhi2019flexible}}
\label{sec:librabft:flexiblebft}
In this section, we compare our OFT-LibraBFT with FBFT~\cite{malkhi2019flexible} which obtains OFT over PBFT but can also be adapted for LibraBFT.
However, the FBFT solution inevitably increases the amortized message complexity from $O(n)$ to $O(n^2)$ per block decision, in contrast to our solution OFT-LibraBFT which keeps the cost linear.

\paragraph{Adapting FBFT to LibraBFT.}
FBFT proposes the notion of flexible BFT quorums, which identifies quorums of different sizes to provide flexible fault tolerance levels for consensus decisions. Although in FBFT~\cite{malkhi2019flexible} only the solution based on PBFT is proposed, it is straightforward to extend the idea of flexible BFT quorums to chain-based BFT SMR protocols such as HotStuff/LibraBFT as well.
The strong commit rule of FBFT on LibraBFT is the following.
% \kartik{mention loss of linearity upfront in this section. Also, the section itself can be moved after the protocol description/analysis.}
% \rl{Agreed. This and next subsections combined take up too much space and reading efforts. In general, I do not like the attempt-problem-attempt2-problem2 style of writing.  
% At a high level, I think we need coordinate the entire paper on how to treat FBFT. My current preference is to consider the goals as different,  the technique FBFT can be modified to achieve strong commit, but not linearly.}

{\bf Strong commit rule (FBFT-LibraBFT).}
    The replica $x$-strong commits a block $B_k$ and all its ancestors, if and only if there exists three adjacent blocks $B_k,B_{k+1},B_{k+2}$ in the chain with consecutive round numbers, 
    and each of $B_k,B_{k+1},B_{k+2}$ has \underline{at least $x+f+1$ distinct signed \vote messages}.
    
Intuitively, the higher level of resilience is achieved by directly increasing the QC size in the $3$-chain rule when strong committing a block. 
The larger QC of a round-$r$ block $B$ consists of more direct \vote messages for $B$ received by the next leader.
However, the protocol loses liveness with QC size larger than $2f+1$, since the number of Byzantine faults may be up to $f$. 
Therefore, replicas should advance to the next round with the standard quorum size of $2f+1$, and any extra \vote messages from earlier rounds need to be multicasted by the leader of that round.
Due to the extra work the leader needs to conduct for every round, the amortized message complexity per round increases in the FBFT approach. 
Since there may be up to $f$ extra votes not included in the QC, the leader may need to multicast up to $f$ extra messages, leading to an amortized message complexity $O(fn)=O(n^2)$ per round and thus $O(n^2)$ per block decision.
% Therefore, adopting the FBFT approach to implement OFT would increase the message complexity from linear to quadratic per block decision, damaging the throughput of the system.
% In contrast, our solution does not require any extra message exchanges, keeping the same message complexity per block decision and throughput as the original LibraBFT protocol.




\subsection{With both round \rmarker and height \hmarker}
\begin{theorem}
    When a block $B$ is $x$-strong committed at some honest replica by the strong commit rule, no other block $B_k'$ at height $k$ can be committed under $t\leq x$ where $t$ is the number of Byzantine faults.
\end{theorem}

\begin{proof}
    Suppose for the sake of  contradiction, under $t\leq x$ Byzantine replicas, a conflicting block $B_k'$ at height $k$ is committed.
    According to the strong commit rule, there exists three blocks $B_k,B_{k+1},B_{k+2}$ with consecutive round numbers $r,r+1,r+2$, and block $B_k$ is $x$-strong committed where
    \[
        x=\min_{l=0,1,2}(|\fn(B_{k+l},\infty,k)\cup \bigcup_{l'\geq l+1} \fn(B_{k+l'}, r+l,k)|)-f-1.
    \]
    
    
    First we prove that any certified block with round number $\geq r$ must extend $B_k$.
    Suppose for the sake of contradiction, it is not true, and let block $B_{k'}'$ be such a certified block with smallest round number $r'\geq r$.
    Then, the parent block of $B_{k'}'$ has round number $<r$, and does not extend $B_k$ as well, otherwise the assumption would be violated.
    Let $A$ denote the set of replicas that certifies $B_{k'}'$ where $|A|=2f+1$.
    Consider the following cases.
    \begin{itemize}
        \item When $r'=r$.  The honest replicas in $A$ will not vote for $B_k$, since honest replicas only vote for one block at each round.
        However, all replicas in $A$ may vote for blocks extending $B_k$, as they are locked on some round number $<r$, and are able to vote for any blocks extending $B_k$ with round number $r$. 
        Recall that $\fn(B_k, r, h)$ denotes the set of signers in the certificate of $B_k$ whose $\rmarker<r$ and $\hmarker<h$, i.e.,
        $\fn(B_k, r, h)=\{i ~|~ \langle \vote, B_k, \marker \rangle_i \in\fc(B_k), \rmarker< r, \hmarker<h\}$.
        Then, any honest replicas in the set $\bigcup_{l'\geq 1} \fn(B_{k+l'}, r, k)$ do not vote for $B_{k'}'$ at round $r$, otherwise their $\marker\geq r$ and should not be included in the set. They also will not vote for $B_{k'}'$ at round $>r$ since they vote in monotonically increasing rounds.
        Therefore, the intersection of set $A$ and set $\bigcup_{l'\geq 1} \fn(B_{k+l'}, r, k)$ contains no honest replicas.
        The above observation implies that the intersection between set 
        $Q=\fn(B_{k}, \infty, \infty)\cup \bigcup_{l'\geq 1} \fn(B_{k+l'}, r, \infty)$
        and set $A$ contains only Byzantine replicas.
        Since the size of intersection is at least $|Q|+|A|-n=|Q|-f$, and $|Q|=|\fn(B_{k}, \infty, \infty)\cup \bigcup_{l'\geq 1} \fn(B_{k+l'}, r, \infty)|\geq =|\fn(B_{k}, \infty, k)\cup \bigcup_{l'\geq 1} \fn(B_{k+l'}, r, k)|\geq x+f+1$, there should be at least $|Q|-f\geq x+f+1-f=x+1$ Byzantine replicas. 
        However, this contradicts the assumptions that there are at most $x$ Byzantine replicas, and therefore $B_{k'}'$ cannot be certified at round $r$.
        
        \item When $r'=r+1$.  Similar to the above case, the honest replicas in $A$ will not vote for $B_{k+1}$, since honest replicas only vote for one block at each round, but they may vote for blocks extending $B_{k+1}$. 
        Therefore the intersection between set 
        $Q=\fn(B_{k+1}, \infty, \infty)\cup \bigcup_{l'\geq 2} \fn(B_{k+l'}, r+1, \infty)$
        and set $A$ contains only Byzantine replicas.
        This implies that there should be at least $|Q|-f\geq x+f+1-f=x+1$ Byzantine replicas, which contradicts the assumptions that there are at most $x$ Byzantine replicas. Therefore $B_{k'}'$ cannot be certified at round $r+1$.
        
        \item When $r'=r+2$. Similar to the cases above, the honest replicas in $A$ will not vote for $B_{k+2}$, since honest replicas only vote for one block at each round, but they may vote for blocks extending $B_{k+2}$. 
        Therefore the intersection between set 
        $Q=\fn(B_{k+2}, \infty, \infty)\cup \bigcup_{l'\geq 3} \fn(B_{k+l'}, r+2, \infty)$
        and set $A$ contains only Byzantine replicas.
        This implies that there should be at least $|Q|-f\geq x+f+1-f=x+1$ Byzantine replicas, which contradicts the assumptions that there are at most $x$ Byzantine replicas. Therefore $B_{k'}'$ cannot be certified at round $r+2$.
        
        \item When $r'\geq r+3$. Since $B_{k+2}$ is certified by the set of replicas in $\fn(B_{k+2}, \infty, \infty)$, the honest replicas in the above set lock on round number $r$ when voting for $B_{k+2}$.
        Then, they will not vote for block $B_{k'}'$ since the parent block of $B_{k'}'$ has round number $<r$.
        Suppose the first block extending $B_{k+2}$ with round number $>r'$ is at height $p$.
        Then the honest replicas in $\bigcup_{k+2\leq j\leq p-1} \fn(B_j, \infty, \infty)$ do not vote for $B_{l'}$ since they are locked on round number $\geq r$.
        However, replicas in $A$ may vote for blocks that extend $B_p$
        Similar to the previous cases, the intersection of $Q=(\cup_{k+2\leq j\leq p-1} \fn(B_j, \infty, \infty)) \bigcup (\cup_{j\geq p} \fn(B_j, r', \infty))$ and the set of replicas that vote for $B_{k'}'$ contains only Byzantine replicas, which implies that there are at least 
        $|Q|-f$ Byzantine replicas. However, since $|Q|-f \geq |\fn(B_{k+2}, \infty, \infty) \bigcup (\cup_{l\geq 3} \fn(B_{k+3}, r', \infty))| - f\geq |\fn(B_{k+2}, \infty, \infty) \bigcup (\cup_{l'\geq 3} \fn(B_{k+l'}, r+2, \infty))| - f \geq |\fn(B_{k+2}, \infty, k) \bigcup (\cup_{l'\geq 3} \fn(B_{k+l'}, r+2, k))| - f \geq x+1$, the number of Byzantine replicas is at least $x+1$. This violates the assumption that $t\leq x$, and thus $B_k'$ cannot be certified at round $\geq r+3$.
        
    \end{itemize}
    Therefore, we proved that any certified block with round number $\geq r$ must extend $B_k$.
    Thus any conflicting height-$k$ block with round number $\geq r$ cannot be committed.
    
    
    Now, consider the case where the round number of $B_k'$ is $<r$. Since $B_k'$ is committed, a set $A$ of $2f+1$ replicas votes for $B_k'$.
    If any honest replica in $A$ votes for $B_k$ or any block extending $B_k$, it will include a $\hmarker\geq k$ in its vote since it voted for a conflicting block $B_k'$ at height $k$.
    Hence, the set $Q=\bigcup_{l\geq 0} \fn(B_{k+l}, \infty, k)$ does not include any honest replica in $A$. 
    Thus the intersection between any of the above set and set $A$ contains only Byzantine replicas.
    This implies that there are at least $|Q|+|A|-n=|Q|-f$ Byzantine replicas.
    Since $\fn(B_{k+l},\infty, k)\cup \bigcup_{l'\geq l+1} \fn(B_{k+l'}, r+l, k)|)\subseteq \bigcup_{l\geq 0} \fn(B_{k+l}, \infty, k)$ for $l=0,1,2$, we have $|Q|\geq \min_{l=0,1,2}|\fn(B_{k+l},\infty, k)\cup \bigcup_{l'\geq l+1} \fn(B_{k+l'}, r+l, k)|)\subseteq \bigcup_{l\geq 0} \fn(B_{k+l}, \infty, k)|=x+f+1$.
    Thus the number of Byzantine replicas is $\geq x+1$, which contradicts the assumption.
    Hence any conflicting $B_k'$ with round number $<r$ cannot be certified.
\end{proof}



\section{LibraBFT with Fast Proposal (similar to HotStuff-Mania)}

In LibraBFT, the leader of each round must wait for $2f+1$ \vote or \timeout messages from the replicas, in order to propose its block.
% In practice, such waiting depends on the slowest sender among the first $2f+1$ messages received, for each round.
A natural question is whether such bottleneck can be removed, by allowing the leader to propose before collecting enough votes.
% A natural idea would be to remove such bottleneck in order to improve the throughput.
Here we propose an intuitively approach to answer the above question affirmatively. 
The idea is to allow the leader of each round $r$ to propose a chain of blocks of the same round number $r$ without waiting or attaching for any votes. 
Meanwhile, the replicas can vote for any of these blocks and send their votes to the next leader.
Once the next leader of round $r+1$ gathers $\geq 2f+1$ distinct endorsements for the first round-$r$ block, it forms a quorum certificate and propose its block of round $r+1$. 
The endorsements can be from votes for any blocks in some prefix $\fp$ of the round $r$ chain, and the first round-$(r+1)$ block should extend $\fp$.

\subsection{Protocol description}

Replicas need to keep a local variable \marker and include \marker in the vote, which equals the {\em largest round number of any block voted on a different branch}.

\begin{itemize}
    
    \item {\bf Endorse.}
    A vote $\langle \vote, B', \marker \rangle_i$ endorses a block $B$ with round number $r$, if (i) $B'=B$ or $B'$ extends $B$, and (ii) $\marker<r$.
    A voter is an endorser of block $B$, if its vote endorses $B$.
    
    \item {\bf $r$-chain ($\fc_r$).} 
    A chain of blocks $B_1,...,B_k$ of round $r$ is call a $r$-chain ($\fc_r$), if the total number of distinct endorsers of $B_1$ is $\geq 2f+1$ from the votes of $B_1,...,B_k$.
    Let the QC of $\fc_r$ be the set of $\geq 2f+1$ distinct votes that endorses $B_1$.
    Let the endorsers of $\fc_r$ be the set of $\geq 2f+1$ distinct endorsers of $B_1$ from the votes of $B_1,...,B_k$.
    
    \item {\bf Proposing rule.}
    The leader of round $r+1$ propose its first round-$(r+1)$ block $B$ when it observes a $\fc_r$ or a \timeout certificate of round $r$. 
    \begin{itemize}
        \item When the leader observes a $\fc_r$, it proposes $B$ that extends $\fc_r$ and contains the QC of $\fc_r$.
        \item When the leader observes a \timeout certificate of round $r$, it proposes $B$ that extends the highest $\fc_{r'}$ in TC (break ties arbitrarily) and contains the TC.
    \end{itemize}
    After proposing the first block, the leader can propose other round-$(r+1)$ blocks extending the last proposed block.
    
    
    \item {\bf Voting rule.} 
    \begin{enumerate}
        \item A replica votes in monotonically {\em non-decreasing} rounds.
        \item A replica votes for a block $B$ if and only if 
        \begin{enumerate}
            \item $B$ of round $r'>r$ directly extends a $\fc_r$ and contains the QC of $\fc_r$ where $r\geq \lock$, or
            \item $B$ of round $r'>r$ contains a \timeout certificate TC, and $B$ directly extends the highest $\fc_r$ in TC where $r\geq \lock$, or
            \item $B$ extends a block $B'$ of the same round number $r$, and $B'$ satisfies one of the above two conditions (a) (b).

        \end{enumerate}
        \item When a replica timeout for round $r$ (not receiving the proposal of round $r+1$ within certain time limit), it broadcasts a \timeout message.
        The \timeout message contains the highest known $\fc_r$ and its QC.
    \end{enumerate}
    
    
    \item {\bf Locking rule.}
    When observing a generalized $2$-chain $\fc_r\fc_{r'}$ in the chain where $r<r'$, 
    a replica sets $\lock = \max(\lock, r)$.
    
    \item {\bf Commit rule.}
    When the chain contains a generalized $3$-chain $\fc_r\fc_{r+1}\fc_{r+2}$ with consecutive round numbers, commit all blocks before $\fc_r$.
    
\end{itemize}


\subsection{Proof of Correctness}
We use $|\fc|$ to denote the number of blocks in $\fc$.
We denote $\fp\preceq \fc$ if $\fp$ is a prefix of $\fc$. 

\subsection*{Safety}

\begin{lemma}\label{fast:lem:1}
    If there exists two $r$-chain $\fc_r$ and $\fc_r'$, then $\fc_r$ and $\fc_r'$ share a common prefix of size $\geq 1$, i.e., $\fp\preceq \fc_r$, $\fp\preceq \fc_r'$ and $|\fp|\geq 1$.
\end{lemma}

\begin{proof}
    Suppose there exists two $r$-chains $\fc_r$ and $\fc_r'$ such that they share no common prefix. Since both $\fc_r$ and $\fc_r'$ have $\geq 2f+1$ endorsers, there exists at least one honest replica that endorses both $\fc_r$ and $\fc_r'$. However, since $\fc_r$ and $\fc_r'$ share no common prefix, they are on different branches. By the definition of endorse, any honest replica cannot endorse both  $\fc_r$ and $\fc_r'$, which is a contradiction.
    Therefore, $\fc_r$ and $\fc_r'$ must share a common prefix of size $\geq 1$.
\end{proof}

\begin{lemma}\label{fast:lem:2}
    % If a $\fc_r$ is directly committed, then any $\fc_{r'}$ with $r'>r$ must extend $\fc_r$.
    If there exists a generalized $3$-chain $\fc_r\fc_{r+1}\fc_{r+2}$ with consecutive round numbers directly extending some block $B$, i.e., $B\fc_r\fc_{r+1}\fc_{r+2}$, then any $\fc_{r'}$ with $r'\geq r$ must extend $B$.
\end{lemma}

\begin{proof}
    Suppose for the sake of contradiction, there exists a $\fc_{r'}$ with $r'\geq r$ that does not extend $B$.
    If $r'=r$ or $r'=r+1$ or $r'=r+2$, by Lemma \ref{fast:lem:1}, $\fc_{r'}$ must share a common prefix with $\fc_r$ or $\fc_{r+1}$ or $\fc_{r+2}$ respectively, and thus must extend $B$.
    Therefore, $r'\geq r+3$. 
    
    Let $\fc_l$ be a chain such that $\fc_{r'}$ extends $\fc_l$ and $\fc_l$ has the smallest round number $l\geq r$. 
    Then the previous $\fc_{l'}$ that $\fc_l$ is directly extending has $l'< r$ by definition.
    If $\fc_l$ extends $B$, then $\fc_{r'}$ also extends $B$, which is a contradiction.
    Therefore $\fc_l$ does not extend $B$. 
    Then by Lemma \ref{fast:lem:1}, we have $l\geq r+3$, otherwise $\fc_l$ will extend $B$.
    At round $l\geq r+3$, at least $2f+1$ replicas have voted for $\fc_{r+2}$ and thus have their $\lock\geq r$ according to the locking rule. 
    Therefore, at least $f+1$ honest replicas that have $\lock\geq r$ will not vote for blocks in $\fc_l$, since $\fc_l$ directly extends $\fc_{l'}$ where $l'< r$.
    Then $\fc_l$ cannot get $2f+1$ endorsers and thus cannot exist, which is a contradiction.
    Therefore, $\fc_{r'}$ must extend $B$.
\end{proof}

\begin{theorem}\label{fast:thm:1}
    If two blocks $B\neq B'$ are both committed, either $B$ extends $B'$ or $B'$ extends $B$.
\end{theorem}

\begin{proof}
    Suppose $B$ is committed due to a generalized $3$-chain $\fc_{r}\fc_{r+1}\fc_{r+2}$,
    and $B'$ is committed due to a generalized $3$-chain $\fc_{r'}\fc_{r'+1}\fc_{r'+2}$.
    Without loss of generality, suppose that $r'\geq r$.
    By Lemma \ref{fast:lem:2}, since $r'\geq r$, $\fc_{r'}$ must extend the block that $\fc_{r}$ is directly extending.
    Therefore, $\fc_{r'}$ must extend $B$, which implies that either $B$ extends $B'$ or $B'$ extends $B$.
\end{proof}


\subsection*{Liveness}


\begin{theorem}
    After GST, if rounds $r,r+1,r+2,r+3$ have honest leaders, then all blocks before $\fc_r$ will be committed.
\end{theorem}

\begin{proof}
    Since the leader of round $r$ is honest, it either proposes the first block extending a $\fc_{r-1}$, or the highest $\fc_{r'}$ in the TC of round $r-1$.
    In the first case, all honest replicas are locked on some $\fc_l$ where $l\leq r-2$, and will vote for the first proposal of round $r$.
    In the second case, let $h$ be the highest \lock that any honest replica has before round $r$.
    This implies this honest replica observes a generalized $2$-chain $\fc_h\fc_{h'}$ where $h'\geq h$, and therefore at least $f+1$ honest replicas have seen $\fc_h$ and voted for $\fc_{h'}$. 
    Therefore, at least one of the $2f+1$ \timeout messages in the round-$r$ TC contains the highest $\fc_l$ where $l\geq h$.
    Hence, the leader in round $r$ is able to propose a block extending $\fc_l$ and containing TC.
    Since all honest replicas have $\lock\leq h\leq l$, they will vote for the proposal of round $r$.
    Then, the leader of round $r$ is able to propose chained blocks of round $r$, and honest replicas will vote for these blocks.
    
    Since the leader of round $r+1$ is honest, when it collects enough \vote messages, it can form a QC for $\fc_r$. Then, based on $\fc_r$, the leader of round $r+1$ can propose its first proposal, and every honest replica will vote for the proposal.
    Similarly, leaders of the following round $r+2$ can propose blocks and form $\fc_{r+2}$. Then, when the first proposal from the leader of round $r+3$ is received by any honest replica, it observes a generalized $3$-chain $\fc_r\fc_{r+1}\fc_{r+2}$ and thus commit any block before $\fc_r$.
    
\end{proof}

\section{LibraBFT without Vote}
Further extending the idea from the previous section, we can obtain the first partially synchronous BFT SMR protocol that does not require any vote.
Only two types of messages are used in the protocol, \proposal and \timeout. 
In the happy path, in each round $r$, the leader of round $r$ broadcasts its \proposal, and rest of the replicas act as followers and broadcast their \proposal's sequentially, extending the longest chain built in round $r$ they have seen.
Once the next leader of round $r+1$ observes a chain of $2f+1$ blocks formed in round $r$, it broadcasts its proposal and make everyone enter round $r+1$.
In the unhappy path, round $r$ will timeout and all replicas will exchange \timeout messages. Then the leader will be replaced when $2f+1$ \timeout messages are gathered.



\subsection{Protocol description}

The protocol proceeds in rounds $r=1,2,...$. In each round, there is a leader that proposes a block first. Then rest of the replicas are called followers in this round, and each of them proposes a block sequentially extending the longest chain it has seen so far.

\begin{itemize}
    
    
    \item {\bf Super block of round $r$ ($\fb_r$).} 
    A chain of blocks $B_1,...,B_k$ of round number $r$ is call a super block of round $r$ ($\fb_r$), if $k\geq 2f+1$ and they are proposed by distinct replicas.
    
    \item {\bf Proposing rule of the leader.}
    The leader of round $r$ proposes its round-$r$ block $B$ when it observes a $\fb_{r-1}$ or a \timeout certificate TC of round $r-1$. 
    \begin{itemize}
        \item When the leader observes a $\fb_{r-1}$, it broadcasts $B$ that extends $\fb_{r-1}$.
        \item When the leader observes a \timeout certificate TC of round $r$, it broadcasts $B$ that extends the highest $\fb_{r'}$ in TC (break ties arbitrarily) and contains the TC.
    \end{itemize}
    
    \item {\bf Proposing rule of other replicas.}
    Assume for each round $r$, there is a predefined order of all replicas starting from the leader.
    When receiving $B_{r-1}$ or TC of round $r-1$, forward and enter round $r$.
    Round $r$ is divided into $n$ iterations, where the $i$-th replica proposes a block in the $i$-th iteration, extending the longest chain it observes.
    A replica enters the $(i+1)$-th iteration when (1) it receives the proposal from the $i$-th replica, or (2) it does not receive the proposal from the $i$-th replica after $2\Delta$ time in iteration $i$.
    
    
    
    \item {\bf Timeout for round.} 
    When a replica enters round $r$, it starts a timer of $2n\Delta$.
    When the timer timeouts before entering round $r+1$, the replica broadcasts a \timeout message for round $r$.
    The \timeout message contains the highest known $\fb_{r'}$ and the proof.
    
    
    \item {\bf Locking rule.}
    When observing a generalized $2$-chain $\fb_r\fb_{r'}$ in the chain where $r<r'$, 
    a replica sets $\lock = \max(\lock, r)$.
    
    \item {\bf Commit rule.}
    When the chain contains a generalized $3$-chain $\fb_r\fb_{r+1}\fb_{r+2}$ with consecutive round numbers, commit all blocks before $\fb_r$.
    
\end{itemize}

\subsection{Proof of Correctness}
\subsection*{Safety}
The safety proof mostly follows from the proof of the earlier section, since the no-vote protocol is a special case of the extension of LibraBFT with fast proposals.
Each $\fb_r$ has blocks proposed by $\geq 2f+1$ distinct replicas, therefore contains $\geq 2f+1$ votes endorsing the first block in $\fb_r$.



\subsection*{Liveness}
\begin{theorem}
    After GST, if rounds $r,r+1,r+2,r+3$ have honest leaders, then all blocks before $\fb_r$ will be committed.
\end{theorem}
\begin{proof}
    The proof also mostly follows from the one for LibraBFT with fast proposals.
    One key observation we can make here is that, after GST, when an honest leader is in charge for round $r$, a $\fb_r$ can be formed.
    First, the leader can propose the first block extending $\bf_{r-1}$ or the highest $\bf_{r'}$ in TC.
    Then all replicas propose their blocks sequentially, extending the longest chain.
    Notice that after every iteration with an honest replica, the length of the longest chain increases by $1$.
    Therefore, after the last honest replica proposes its block, the length of the chain with round-$r$ blocks is $\geq 2f+1$. Then the leader of the next round will receive $\fb_{r}$, and propose the first block in round $r+1$.
\end{proof}








\begin{comment}
\section{A Responsive Protocol with Optimistic Fault Tolerance}

The protocol is presented in Figure \ref{fig:smr}, which is leader-based with rotating leaders.
For efficiency purpose, we let each leader's duration to be $5$ consecutive rounds, i.e., the first leader is in charge of round $1-5$, the second leader is in charge of round $6-10$ and so on.
Every replica keeps a variable \marker locally, which is the highest height of a block on a different branch that the replica ever voted for.


\begin{figure}[h!]
    \centering
    \begin{mybox}
    \textbf{Protocol for Replica $i$}

Let $L_r$ be the leader of round $r$. Initially, every replica set $\lock=0$, and set $\marker=0$.
For asynchronous round $r=1,2,...$, perform the following.
\begin{itemize}
    \item\label{smr:propose} {\bf Propose.} 
    After receiving $2f+1$ distinct signed \vote or \timeout messages from round $r-1$, the leader $L_r$ sends $\langle \texttt{propose}, B_k \rangle_{L_r}$ to all other replicas, 
    where $B_k=(b_k, r, h_{k-1})$ is a height-$k$ block, containing a batch of new client requests $b_k$ and a hash digest $h_{k-1}=H(B_{k-1})$ of block $B_{k-1}$, where $B_{k-1}$ is the last block of the longest certified chain known to the leader.
    
    \item\label{smr:vote} {\bf Vote.} 
    Upon receiving the first valid proposal $\langle \texttt{propose}, B_k\rangle_{L_r}$ at round $r$, 
    send a \vote to all other replicas~\footnote{The protocol can be changed to sending to vote only to the next leader. Then the protocol need additional steps for out-of-sync replicas to fetch missing blocks.}
    in the form of $\langle \vote, B_k, \marker \rangle_i$ if (1) the replica has seen the certified parent chain $B_1\cdots B_{k-1}$, and (2) the replica has not seen a certified chain of length $k+1$.
    Stop the \timeout timer for round $r-1$ and start the \timeout timer for round $r$.
    Stop voting for round $r-1$.
    
    \item\label{smr:timeout} {\bf Timeout.}
    Upon timeout at round $r$, send a \timeout to all other replicas in the form of $\langle \timeout, B_k, \marker \rangle_i$, where $B_k$ is the first valid proposal received at round $r$, or $B_k=(\bot, r, h_{k-1})$ and $h_{k-1}=H(B_{k-1})$ where $B_{k-1}$ is the last block of the longest certified chain known to the leader, if no valid proposal is received.
    
    Upon receiving $2f+1$ \timeout messages from round $r-1$, 
    stop the \timeout timer for round $r-1$ and start the \timeout timer for round $r$.
    Stop voting for round $r-1$.

    % \item\label{smr:lock} {\bf Lock.} 
    % When observing a certified chain $B_1\cdots B_kB_{k+1}$ while having $\lock=B_{k'}$ and $k'<k$, update $\marker$ if $B_k$ does not extend $\lock$, and
    % update $\lock = B_k$.
    
    
    \item\label{smr:commit} {\bf Regular Commit.} 
    When observing a certified chain $B_1\cdots B_{k-2}B_{k-1}B_kB_{k+1}B_{k+2}$ such that the last $5$ blocks $B_{k-2}B_{k-1}B_kB_{k+1}B_{k+2}$ have consecutive round numbers, then prefix $B_1\cdots B_k$ is committed.
    
    \item\label{smr:strongcommit} {\bf Strong Commit.}
    When observing a certified chain $B_1\cdots B_{k-2}B_{k-1}B_kB_{k+1}B_{k+2}\cdots$ that contains $5$ blocks $B_{k-2},B_{k-1},B_k,B_{k+1},B_{k+2}$ with consecutive round numbers, then the block $B_k$ is $x$-strong committed, where
    \[
        x=\min_{k-2\leq l\leq k+2}(|\fn(B_l,\infty)\cup \bigcup_{l'\geq l+1} \fn(B_{l'}, k)|)-f-1.
    \]
    $\fn(B_l, k)$ is the set of signers in the certificate of $B_l$ whose $\marker<k$, i.e.,
    $\fn(B_l, k)=\{i ~|~ \langle *, B_l, \marker \rangle_i \in\fc(B_l), \marker< k\}$.
    $\fn(B_l, \infty)$ is the set of all signers in the certificate of $B_l$.
    \end{itemize}

    \end{mybox}
    \caption{BFT SMR with optimistic fault tolerance}
    \label{fig:smr}
\end{figure}


\section{Proof of Correctness}

\subsection{Safety for regular commit}
When proving the safety for regular commit, we assume the number of Byzantine faults $t\leq f$ where $n=3f+1$.
\begin{lemma}\label{lemma:safety1:1}
    Two different blocks cannot both be certified at the same round.
\end{lemma}
\begin{proof}
    Since honest replicas only vote for the first valid block in every round, due to quorum intersection only one block can be certified for each round.
\end{proof}

\begin{lemma}\label{lemma:safety1:2}
    If a height-$k$ block $B_k$ is committed at some honest replica, no other height-$k$ block $B_k'$ can be certified.
\end{lemma}
\begin{proof}
    Suppose that block $B_k$ is committed at honest replica $h$. According to the commit rule, $h$ has observed a chain of certified blocks ending with $B_{k-2}B_{k-1}B_kB_{k+1}B_{k+2}$, and $B_{k-2},B_{k-1},B_k,B_{k+1},B_{k+2}$ have consecutive round numbers, i.e., $r-2,r-1,r,r+1,r+2$ respectively.
    Suppose for the sake of contradiction, another height-$k$ block $B_k'$ is certified. 
    Let $r'$ denote the round number of $B_k'$. Consider the following cases:
    \begin{itemize}
        \item When $r'<r-2$. Since $B_k'$ is proposed at round $r'<r-2$ and gets certified, at least $f+1$ honest replicas voted for $B_k'$ at round $r'<r-2$. Let $B_{k-2}'$ denote the height-$k-2$ block that $B_k'$ extends. It is clear that $B_{k-2}'\neq B_{k-2}$, since $B_{k-2}$ is not yet proposed in round $r'$.
        According to the voting rule, all the above $f+1$ honest replicas seen a certified length-$(k-1)$ parent chain of $B_k'$ when voting for $B_k'$. The above honest replica  at round $r-2$ will not vote for $B_{k-2}$ they have seen a certified chain of length $k-1$. 
        Therefore, $B_{k-2}$ cannot be certified, which contradicts the assumption.
        Thus $B_k'$ cannot be certified.
        
        \item When $r-2\leq r'\leq r+2$. By Lemma \ref{lemma:safety1:1}, no two different blocks can be certified at the same round. Since $B_{k-2},B_{k-1},B_k,B_{k+1},B_{k+2}$ are certified, $B_k'$ cannot be certified.
        
        \item When $r'>r+2$. Since $B_{k+2}$ is certified at round $r+2$, at least $f+1$ honest replicas voted for $B_{k+2}$ and have seen the certified parent chain $B_1\cdots B_{k+1}$. According to the voting rule, they will not vote for $B_k'$ later, and thus $B_k'$ cannot be certified.
        
    \end{itemize}
\end{proof}

\begin{theorem}
    Honest replicas always commit the same block $B_k$ for each height $k$.
\end{theorem}
\begin{proof}
    Consider any two blocks $B_k$ and $B_k'$ committed at height $k$ at honest replicas. Let $B_k$ be committed due to a height-$l$ block $B_l$ being directly committed. Let $B_k'$ be committed due to a height-$l'$ block $B_{l'}'$ being directly committed. 
    Without loss of generality, suppose that $l\leq l'$. 
    By Lemma \ref{lemma:safety1:2}, when $B_l$ is committed, no other height-$l$ block can be certified. Therefore $B_{l'}'$ must extend $B_l$, and thus $B_k=B_k'$.
\end{proof}
\subsection{Safety for strong commit}

\begin{theorem}
    When a height-$k$ block $B_k$ is $x$-strong committed at some honest replica by the strong commit rule, no other height-$k$ block $B_k'$ can be committed under $t\leq x$ where $t$ is the number of Byzantine faults.
\end{theorem}
\begin{proof}
    Recall that $\fn(B_l, k)$ denotes the set of signers in the certificate of $B_l$ whose $\marker<k$, i.e.,
    $\fn(B_l, k)=\{i ~|~ \langle *, B_l, \marker \rangle_i \in\fc(B_l), \marker< k\}$. 
    Then $\fn(B_l, \infty)$ denotes the set of all signers in the certificate of $B_l$.
    
    Suppose that block $B_k$ is $x$-strong committed at honest replica $h$. According to the strong commit rule, $h$ has observed a chain of certified blocks ending with $B_{k-2}B_{k-1}B_kB_{k+1}B_{k+2}$, and $B_{k-2},B_{k-1},B_k,B_{k+1},B_{k+2}$ have consecutive round numbers, i.e., $r-2,r-1,r,r+1,r+2$ respectively. What's more, the value of $x$ satisfies that $x=\min_{k-2\leq l\leq k+2}(|\fn(B_l,\infty)\cup \bigcup_{l'\geq l+1} \fn(B_{l'}, k)|)-f-1$, where
    $\fn(B_l, k)$ is the set of signers in the certificate of $B_l$ whose $\marker<k$, i.e.,
    $\fn(B_l, k)=\{i ~|~ \langle *, B_l, \marker \rangle_i \in\fc(B_l), \marker< k\}$.
    Suppose for the sake of contradiction, another height-$k$ block $B_k'$ is committed under $t\leq x$.
    Then block $B_k'$ must be certified as well.
    Let $r'$ denote the round number of $B_k'$. Consider the following cases:
    \begin{itemize}
        \item When $r'< r-2$. Since $B_k'$ is proposed at round $r'\leq r-2$ and gets certified, a set $A$ of at least $2f+1-t$ honest replicas voted for $B_k'$ at round $r'$. 
        Suppose $B_{k-2}',B_{k-1}',B_k'$ are the last $3$ blocks of the chain seen by the honest replicas when they vote for $B_k'$, where $B_{k-2}',B_{k-1}'$ are proposed before round $r'$.
        According to the voting rule, all honest replicas in $A$ have seen the certified length-$(k-1)$ parent chain of $B_k'$ when voting for $B_k'$. 
        By the voting rule, the honest replicas in $A$ will not vote for blocks $B_{k-2}$.
        Hence the set of replicas $\fn(B_{k-2}, \infty)$ that vote for blocks $B_{k-2}$ contains no honest replicas in $A$.
        However, when the honest replicas in $A$ receives block $B_l$ where $l\geq k-1$, they may vote for $B_l$ since they haven't seen a certified chain of length $k$.
        By the definition of $\fn(B_l, k)$, $\bigcup_{l\geq k-1} \fn(B_l, k)$ is the union of the set of honest replicas that do not vote for $B_k'$ but vote for some block $B_l$ where $l\geq k-1$, and a subset of Byzantine replicas.
        Therefore, 
        $Q=(\fn(B_{k-2}, \infty)\bigcup (\cup_{l\geq k-1} \fn(B_l, k))$ contains no honest replicas in $A$.
        Thus, the intersection of $Q$ and the set of replicas that vote for $B_k'$ contains only Byzantine replicas, which implies that there are at least 
        $|Q|+2f+1-n=|Q|-f$ Byzantine replicas. However, since $|Q|-f\geq |\fn(B_k,\infty)\bigcup(\cup_{l\geq k+1} \fn(B_l, k))|-f\geq x+1$, the number of Byzantine replicas is at least $x+1$. This violates the assumption that $t\leq x$, and thus $B_k'$ cannot be certified.
        
        
        \item When $r-2\leq r'\leq r+2$. Consider the case when $r'=r+a$ where $-2\leq a \leq 2$. The honest replicas that vote for block $B_k'$ will not vote for $B_{k+a}$, since $B_{k+a}$ is also proposed in round $r'$. Similar to the previous case, when the above honest replicas receives block $B_l$ where $l\geq k+a+1$, they vote for $B_l$ since they haven't seen a certified chain of length $k+a+2$. 
        Hence, $Q=( \fn(B_{k+a}, \infty)\bigcup (\cup_{l\geq k+a+1} \fn(B_l, k))$ contains no honest replicas that vote for $B_k'$.
        Thus, the intersection of $Q$ and the set of replicas that vote for $B_k'$ contains only Byzantine replicas, which implies that there are at least 
        $|Q|-f$ Byzantine replicas. However, since $|Q|-f\geq x+1$, the number of Byzantine replicas is at least $x+1$. This violates the assumption that $t\leq x$, and thus $B_k'$ cannot be certified.
        
        \item When $r'\geq r+3$.  When any honest replica votes for block $B_{k+2}$ at round $r+2$, they have seen a certified chain of length $k+1$. Thus, it will not vote for $B_k'$ according to the voting rule.
        Similarly for any block $B_{k'}$ extending $B_{k+2}$ with round number $\leq r'$, any honest replica that votes for $B_{k'}$ has seen a length-$(k'-1)$ certified chain and will not vote for $B_k'$ at round $r'$.
        Suppose the first block extending $B_{k+2}$ with round number $>r'$ is at height $h$.
        Then the honest replicas in $\bigcup_{k+2\leq l\leq h-1} \fn(B_l, \infty)$ do not vote for $B_{k'}$.
        By the definition of $\fn(B_l, k)$, $\bigcup_{l\geq h} \fn(B_l, k)$ is the union of the set of honest replicas that do not vote for $B_k$ but vote for some block $B_l$ where $l\geq h$ at round $> r'$, and a subset of Byzantine replicas.
        Therefore, the intersection of $Q=(\cup_{k+2\leq l\leq h-1} \fn(B_l, \infty)) \bigcup (\cup_{l\geq h} \fn(B_l, k))$ and the set of replicas that vote for $B_k'$ contains only Byzantine replicas, which implies that there are at least 
        $|Q|-f$ Byzantine replicas. However, since $|Q|-f=|(\cup_{k+2\leq l\leq h-1} \fn(B_l, \infty)) \bigcup (\cup_{l\geq h} \fn(B_l, k))|-f\geq |(\fn(B_{k+2}, \infty) \bigcup (\cup_{l\geq k+3} \fn(B_l, k))| - f \geq x+1$, the number of Byzantine replicas is at least $x+1$. This violates the assumption that $t\leq x$, and thus $B_k'$ cannot be certified.
    \end{itemize}
\end{proof}


\subsection{Liveness}

Suppose the timeout is large enough for a round to finish under an honest leader. 
Suppose the number of Byzantine replicas is $t\leq f$.
\begin{theorem}
    After GST, honest replicas keep committing new blocks.
\end{theorem}

\begin{proof}
    First, the leader rotates within a finite time due to the \timeout scheme. We will prove that once an honest leader is in charge of $5$ consecutive rounds, new blocks will be committed at honest replicas. Therefore, all honest replicas keep committing new blocks when honest leaders is in charge.
    
    Suppose an honest leader $L$ is in charge of rounds $r$ to $r+4$. 
    Before $L$ sends its proposal, it wait for $2f+1$ \vote or \timeout messages from round $r-1$, which will eventually happen since there are $\leq f$ Byzantine replicas.
    Let chain $B_1\cdots B_k$ be the longest certified chain that any honest replica has seen before round $r$.
    Therefore, at least $f+1$ honest replicas voted for $B_k$ before round $r$, and thus have seen a certified chain $B_1\cdots B_{k-1}$.
    Then, at least one \vote or \timeout message received by $L$ is from the above $f+1$ honest replicas, which carries $B_{k-1}$. 
    Thus the leader $L$ will propose a block extending $B_{k-1}$, and all honest replica will vote for the proposal.
    The leader $L$ is then able to continue and propose $5$ blocks in total with consecutive round numbers and all blocks can be certified by the honest replicas.
    Therefore, according to the commit rule, $3$ out of $5$ blocks are committed.
\end{proof}




\end{comment}






